Infrared Emission of Specific Polycyclic Aromatic Hydrocarbon Molecules: Cyanonaphthalenes

The unidentified infrared emission (UIE) features at 3.3, 6.2, 7.7, 8.6, 11.3 and 12.7 micron are ubiquitously seen in a wide variety of astrophysical regions and commonly attributed to polycyclic aromatic hydrocarbon (PAH) molecules. However, the unambiguous identification of any individual, specific PAH molecules has proven elusive until very recently two isomers of cyanonapthalene, which consists of two fused benzene rings and substitutes a nitrile (-CN) group for a hydrogen atom, were discovered in the Taurus Molecular Cloud based on their rotational transitions at radio frequencies. To facilitate the James Webb Space Telescope (JWST) to search for cyanonapthalenes in astrophysical regions, we model the vibrational excitation of cyanonapthalenes and calculate their infrared emission spectra in a number of representative astrophysical regions. The model emission spectra and intensities will allow JWST to quantitatively determine or place an upper limit on the abundance of cyanonapthalenes.

==> abstract.tex <==

Infrared Emission of Specific Polycyclic Aromatic Hydrocarbon Molecules: Cyanonaphthalenes


The unidentified infrared emission (UIE) features at 3.3, 6.2, 7.7, 8.6, 11.3 and 12.7 micron are ubiquitously seen in a wide variety of astrophysical regions and commonly attributed to polycyclic aromatic hydrocarbon (PAH) molecules. However, the unambiguous identification of any individual, specific PAH molecules has proven elusive
until very recently two isomers of cyanonapthalene, which consists of two fused benzene rings and substitutes a nitrile (–CN) group for a hydrogen atom, were discovered in the Taurus Molecular Cloud based on their rotational transitions at radio frequencies. To facilitate the James Webb Space Telescope (JWST) to search for cyanonapthalenes in astrophysical regions, we model the vibrational excitation of cyanonapthalenes and calculate their infrared emission spectra in a number of representative astrophysical regions. The model emission spectra and intensities will allow JWST to quantitatively determine or place an upper limit on the abundance of cyanonapthalenes.
